Detecting Data Poisoning in Code Generation LLMs via Black-Box, Vulnerability-Oriented Scanning

Code generation large language models (LLMs) are increasingly integrated into modern software development workflows. Recent work has shown that these models are vulnerable to backdoor and poisoning attacks that induce the generation of insecure code, yet effective defenses remain limited. Existing scanning approaches rely on token-level generation consistency to invert attack targets, which is ineffective for source code where identical semantics can appear in diverse syntactic forms. We present CodeScan, the first black-box, vulnerability-specific scanning framework for auditing code generation LLMs, assuming that the defender specifies the target vulnerability classes and provides corresponding task-relevant prompts. CodeScan identifies attack targets by analyzing structural similarities across multiple generations conditioned on different clean prompts. It combines iterative divergence analysis with abstract syntax tree (AST)-based normalization to abstract away surface-level variation and unify semantically equivalent code, isolating structures that recur consistently across generations. CodeScan then applies LLM-based vulnerability analysis to determine whether the extracted structures contain security vulnerabilities and flags the model as compromised when such a structure is found. We evaluate CodeScan against four representative attacks under both backdoor and poisoning settings across three real-world vulnerability classes. Experiments on 117 models spanning three architectures and multiple model sizes demonstrate 97%+ detection accuracy with substantially lower false positives than prior methods.

==> discussion.tex <==
\section{Discussion}

%\YH{CodeScan assumes known vulnerability classes, representative task-relevant prompts, a reliable vulnerability analyzer, and a sufficiently consistent structural signal. It may miss unknown vulnerabilities, behavior outside the supplied prompts, structurally diversified targets, and stronger adaptive attacks. }

%\vspace{0.02in}

% \noindent\textbf{More Complex Attack Targets.}
% Our current evaluation focuses on relatively short and self-contained vulnerable attack target, which is aligned with all existing poisoning attacks, such as \simple, \covert, \trojanpuzzle, \codebreaker. For more complex attack targets, such as those spanning multiple functions or involving subtle data-flow vulnerabilities (e.g., use-after-free), the effectiveness of \ours depends on whether the poisoned model can still generate a sufficiently consistent attack target with high probability once the first target token is reached. If the backdoor causes the model to reliably produce such multi-line or multi-function vulnerable patterns, then the same intuition underlying \ours still applies: structurally biased generations can be identified through divergence analysis and subsequently verified by vulnerability analysis. However, if the target is highly dispersed, weakly triggered, or only manifests through long-range semantic interactions rather than recurring structural patterns, firstly I think the attacker won't use it, because they should guarantee the attack success.
% then both inversion and structural clustering become more challenging. In such cases, \ours may require richer program representations beyond line-level ASTs, such as inter-procedural structure or data-flow information, which we leave to future work.

% \YSA{add a discussion on the generalibility of CodeScan to other attacks, including BadEdit.}

% \YSA{\noindent\textbf{Generalizability to Other Attacks.} \ours is designed to detect backdoors in poisoned code LLMs, but it can also be applied to attacks originally proposed for general-purpose LLMs, as long as they can be adapted to code LLMs. 
% For example, we adapted BadEdit~\cite{li2024badedit} to CodeLlama by using our V1 text trigger with the simple-attack target.
% \ours successfully detects the resulting backdoor.
% Moreover, its black-box detection mechanism could potentially be extended to other attack settings, such as indirect prompt injection~\cite{greshake2023not}, malicious retrieval contexts~\cite{zou2025poisonedrag}, and compromised agent/tool workflows.}

% \vspace{0.02in}


\noindent\textbf{More Complex Attack Targets.}
Our evaluation focuses on relatively short and self-contained attack targets, consistent with all existing attacks such as \codebreaker. 
For more complex targets spanning multiple functions or involving subtle data-flow vulnerabilities, \ours depends on whether the poisoned model can still generate the attack target pattern consistently. 
% If so, the same intuition behind \ours still applies: structurally biased generations can be identified through divergence analysis and then verified by vulnerability analysis. 
If so, \ours can identify structurally biased generations through divergence analysis and verify them via vulnerability analysis. 
Otherwise, inversion and structural clustering become more challenging. 
In practice, such weak or dispersed targets may also be less attractive to attackers because they reduce attack reliability. 
Handling these cases may require richer program representations, such as inter-procedural structure or data-flow information, which we leave to future work.




% \vspace{0.05in}
% \noindent\textbf{Impact of the Vulnerability Analyzer.}
% The vulnerability analysis component in Step~2 is modular and separate from Step~1. Step~1 is responsible for narrowing the search space by identifying structurally consistent attack-target candidates without knowing the trigger, while Step~2 determines whether these candidates actually contain the vulnerability under consideration. Therefore, with a stronger analyzer, it would primarily improve the precision of Step~2 by reducing false positives, and may also improve recall by identifying more subtle vulnerable patterns. Conversely, using a weaker analyzer would mainly degrade the performance of Step~2, potentially increasing both false positives and false negatives. However, compared with \bait, the key advantage of \ours lies in Step~1: \ours produces substantially more precise attack-target candidates through structural divergence analysis, whereas \bait relies only on token-level bias signals and thus yields many spurious candidates. Moreover, \bait+VA is better than \bait and worse than \ours, so weaker analyzer also weaks \bait+VA. As a result, even though the absolute performance of \ours depends on the strength of the analyzer used in Step~2, its candidate quality remains consistently better than that of \bait+VA, \bait and related baselines.

\vspace{0.02in}

\noindent\textbf{Impact of the Vulnerability Analyzer.}
The vulnerability analyzer in Step~2 is modular and separate from Step~1. Step~1 narrows the search space by identifying structurally consistent candidates, while Step~2 determines whether they contain the target vulnerability. A stronger analyzer can improve Step~2 by reducing false positives and false negatives, whereas a weaker analyzer may have the opposite effect. However, CodeScan’s main advantage over \bait lies in Step~1: structural divergence analysis produces cleaner candidates, whereas \bait relies only on token-level bias signals and yields many spurious candidates. Since BAIT+VA uses the same analyzer-dependent Step~2, weaker analyzers also degrade its performance. Thus, although CodeScan’s absolute performance depends on the analyzer used in Step~2, it is still expected to outperform BAIT+VA, \bait, and related baselines under the same analyzer.



% \YSA{"How would CodeScan handle attack targets that span multiple functions or involve subtle data-flow vulnerabilities (e.g., UAF) rather than localized API misuse patterns? The current evaluation focuses on relatively short, self-contained vulnerable code snippets. Thus I am wondering does the structural divergence analysis scale to more complex attack targets?"
% Add discussion for this. For more complex attack targets, maybe the attack cannot generate it. If it can, based on our experiments design, as long as the model can generate the attack target with high rate, we can invert it. }

% \textbf{Vulnerability-specific Probing.}
% \ours focuses on vulnerability specific model probing rather than exhaustive vulnerability detection in real-world software. In practice, defenders rarely attempt to enumerate the full vulnerability space; instead, they prioritize a small set of high-impact, well-understood vulnerability classes that pose immediate security risks. This formulation mirrors vulnerability-specific static analysis rules or queries~\cite{pearce2025asleep, fu2025security}.
% % , which likewise assume a finite and predefined vulnerability scope~\cite{pearce2025asleep, fu2025security}.
% Importantly, \ours is designed to probe known vulnerability classes rather than to discover zero-day vulnerabilities. This aligns with realistic threat models, as poisoning attacks typically exploit established vulnerabilities for reliable activation, and defenders monitor for such patterns during model auditing.
% Rather than exhaustively detecting vulnerabilities in generated code, \ours aims to assess whether a model has been behaviorally compromised, offering a practical and complementary approach to evaluating the trustworthiness of code generation models.
% \ours focuses on vulnerability-specific model probing rather than comprehensive vulnerability detection in real-world software. In practice, security workflows rarely attempt to enumerate the entire vulnerability space; instead, defenders typically prioritize a small set of high-impact and well-understood vulnerability classes—such as hard-coded credentials, disabled certificate verification, or command injection—that pose immediate and severe security risks. Within this setting, our approach can be viewed as a targeted probing mechanism: given a vulnerability hypothesis of interest, the defender evaluates whether a target model has been maliciously biased toward generating code that exhibits the corresponding weakness. This formulation is analogous to vulnerability-specific static analysis rules or queries, which likewise operate under a finite and predefined vulnerability scope~\cite{pearce2025asleep, fu2025security}.

% Importantly, \ours is primarily designed to probe existing or known vulnerability classes, rather than to discover previously unknown (zero-day) vulnerabilities. This design choice reflects realistic defensive practice: poisoning and backdoor attacks typically exploit known vulnerability patterns to ensure reliable activation, and defenders correspondingly monitor for such patterns during model evaluation and auditing. Moreover, \ours aims to determine whether a model has been compromised at the behavioral level, rather than to perform exhaustive vulnerability detection on generated code. We believe such vulnerability-specific probing represents a practical and complementary approach for assessing the trustworthiness of code generation models under realistic defensive constraints.





% \vspace{0.05in}

% \noindent\textbf{Other Baselines.}
% As discussed in the \bait, several discrete gradient-based optimization or search methods—such as GCG~\cite{zou2023universal}, GDBA~\cite{guo2021gradient}, PEZ~\cite{wen2023hard}, UAT~\cite{wallace2019universal}, and DBS~\cite{feng2023detecting}—can in principle be considered as alternative baselines. 
% However, as reported in \bait, when applied to LLMs, the underlying objective function exhibits severe non-smoothness and oscillatory behavior during optimization. 
% % This instability prevents reliable convergence and makes these methods ineffective at consistently recovering either the trigger or the target sequence. 
% Empirical results~\cite{shen2025bait} show that their performance is already substantially inferior to token-based autoregressive inversion methods such as \bait. 
% Therefore, in this work, we do not include these approaches as baselines.
% % and instead focus on a detailed comparison between \ours and \bait, which represents the strongest and most relevant prior method under the same problem formulation.


% \vspace{0.05in}

% \noindent\textbf{Scope of Vulnerability Transformations and Obfuscation.} 
% In our vulnerability analysis dataset, we consider the same 15 vulnerabilities studied in \codebreaker. Our results show that GPT-5–level models can reliably detect vulnerable code designed to evade GPT-4–based detectors; accordingly, we do not introduce additional vulnerability types. We also do not apply further transformations or obfuscation targeting GPT-5. Given GPT-5’s strong detection capability, the transformation strategy in \codebreaker is no longer directly applicable, and designing more advanced evasion techniques against state-of-the-art analyzers is beyond the scope of this work.


\vspace{0.02in}


\noindent\textbf{Scope of Vulnerability Transformations and Obfuscation.}
Our vulnerability analysis dataset covers the same 15 vulnerabilities studied in \codebreaker. Results show that GPT-5–level models can reliably detect code crafted to evade GPT-4–based detectors; thus, we do not introduce additional vulnerability types. We also do not apply further obfuscation targeting GPT-5. Given its strong detection capability, \codebreaker’s transformation strategy is no longer effective, and developing more advanced evasion techniques against state-of-the-art analyzers is beyond the scope of this work.





% \noindent\textbf{Attack Targets Not Beginning on a New Line.}
% Our experiments consider attack targets that begin on a new line, as shown in \autoref{fig:payloads}. 
% However, \ours is not limited to this setting and can also be applied when the payload does not start at a new line. 
% For example, consider the case where the attack target is \texttt{verify=False} in the statement \texttt{requests.get(url, verify=False)}. 
% If the first token of the payload, \texttt{verify}, is concatenated to the prefix \texttt{requests.get(url, }, the attacked model can subsequently generate the remaining payload \texttt{=False}. 
% This demonstrates that \ours can successfully recover and probe attack targets that appear inline within existing statements, rather than only those introduced as standalone lines.

\vspace{0.02in}

\noindent\textbf{Attack Targets Not Beginning on a New Line.}
Our experiments consider attack targets that begin on a new line, as shown in \autoref{fig:payloads}. 
% However, \ours also applies when the payload does not start on a new line. 
However, \ours also applies to inline payloads. 
For example, if the target is \texttt{verify=False} in \texttt{requests.get(url, verify=False)}, concatenating its first token, \texttt{verify}, to the prefix \texttt{requests.get(url, } can cause the attacked model to generate the remaining \texttt{=False}. 
This shows that \ours can recover inline attack targets within statements, not only standalone-line payloads.




%\YH{Discuss/clarify the support on more vulnerabilities, especially existing vulnerabilities vs zero-day vulnerability} \YSA{added to the first bullet}


% 1. on larger models

% 2. correlation between ASR and inversion rate

% 1. vulnerabilities cases are not comprehensive (in vulnerability detection)

% 2. efficiency (For checking N vulnerabilities)

% 3. What if the payload is not from the beginning of one line.

% 4. other baselines 


